Detection and Isolation of Link Failures under the Agreement Protocol

In this paper a property of the multi-agent consensus dynamics that relates the failure of links in the network to jump discontinuities in the derivatives of the output responses of the nodes is derived and verified analytically. At the next step, an algorithm for sensor placement is proposed, which would enable the designer to detect and isolate any link failures across the network based on the observed jump discontinuities in the derivatives of the responses of a subset of nodes. These results are explained through elaborative examples.

==> omittext.tex <==
it follows that, $\forall \mathscr{W}$ $\in$ $\Omega^{m}(\tilde{\mathscr{G}}_1;{s,k})$ $\cup$ $\Omega^{m}(\tilde{\mathscr{G}}_2;{s,k})$ and $s$ $\not\in$ $\{i,j\}$, $\omega(\mathscr{W},-\mathscr{L}(\mathscr{G}_1))$ $=$ $\omega(\mathscr{W},-\mathscr{L}(\mathscr{G}_2))$, hence

==> omittext2.tex <==
$\{ \mathscr{W} $ $\in$ $ \Omega^{m}(\tilde{\mathscr{G}}_1;{\nu_s,\nu_k}); (\nu_j,\nu_i)$ $\in$ $ \mathscr{W}  \}$ $=$ $\varnothing$, i.e. 





$\Phi(\Omega^{m}(\tilde{\mathscr{G}}_1);{\nu_i,\nu_i,\nu_k}))$ $=$ $(-{d}^{-}_{\mathscr{G}_1}\{\nu_i\})$ $\textrm{c}_{m-1}(\mathscr{G}_1;{\nu}_i,{\nu}_k)$ and $\Phi(\Omega^{m}(\tilde{\mathscr{G}}_2;{\nu_i,\nu_i,\nu_k}))$ $=$ $(-{d}^{-}_{\mathscr{G}_2}\{\nu_i\})$ $\textrm{c}_{m-1}(\mathscr{G}_1;{\nu}_i,{\nu}_k)$ $=$ $(-{d}^{-}_{\mathscr{G}_1}\{\nu_i\} + 1)$ $\textrm{c}_{m-1}(\mathscr{G}_1;{\nu}_i,{\nu}_k)$, so that \eqref{eq:sumWeightsIJpartitioned2} simplifies into $\nabla_i(m)$ $=$ $-\textrm{c}_{m-1}(\mathscr{G}_1;{\nu}_i,{\nu}_k){x}_i(0)$.
